Linear Aggregation in Tree-based Estimators

Regression trees and their ensemble methods are popular methods for nonparametric regression: they combine strong predictive performance with interpretable estimators. To improve their utility for locally smooth response surfaces, we study regression trees and random forests with linear aggregation functions. We introduce a new algorithm that finds the best axis-aligned split to fit linear aggregation functions on the corresponding nodes, and we offer a quasilinear time implementation. We demonstrate the algorithm's favorable performance on real-world benchmarks and in an extensive simulation study, and we demonstrate its improved interpretability using a large get-out-the-vote experiment. We provide an open-source software package that implements several tree-based estimators with linear aggregation functions.

==> 5-ConfidenceIntervals.tex <==
\section{Confidence Intervals} \label{section:confidenceIntervals}

==> X_7-Stopping_criterion.tex <==
\section{A Note on the Early Stopping Algorithm}

As regression trees have been known to have a propensity to overfit when grown to purity, it is common to prune the leaves of the tree either during or after training.
[[Need some citations here]]

In the case of Linear Regression Trees, the linear aggregation functions both allow and require larger leaf nodes compared to standard CART trees.
In order to select final node sizes in a data driven way, we introduce the early stopping algorithm (presented in detail in Algorithm \ref{algo:EarlyStopping}).
The early stopping algorithm considers the $R^2$

==> tables/hyperparameters.tex <==
% latex table generated in R 3.5.0 by xtable 1.8-3 package
% Thu May 30 00:52:05 2019

\begin{table}[!ht]
\begin{flushleft}
\begin{tabular}{rrrrrr}
  \hline
Dataset & mtry & nodesizeSpl & overfitPenalty & LOGminSplitGain & sample.fraction \\ 
  \hline
Friedman 1 & 9 & 16 & 0.23 & -3.86 & 0.91 \\ 
  Friedman 2 & 3 & 195 & 0.43 & -5.07 & 0.89 \\ 
  Friedman 3 & 4 & 11 & 6.65 & -3.16 & 0.65 \\ 
  Boston Housing fold1 & 10 & 7 & 0.28 & -7.86 & 0.95 \\ 
  Boston Housing fold2 & 4 & 13 & 3.06 & -4.81 & 0.99 \\ 
  Boston Housing fold3 & 3 & 12 & 0.19 & -4.94 & 0.94 \\ 
  Boston Housing fold4 & 5 & 13 & 0.77 & -9.12 & 0.91 \\ 
  Boston Housing fold5 & 2 & 11 & 0.25 & -13.71 & 0.99 \\ 
  Ozone fold1 & 2 & 19 & 9.47 & -6.41 & 0.5 \\ 
  Ozone fold2 & 3 & 12 & 3.06 & -4.81 & 0.99 \\ 
  Ozone fold3 & 1 & 20 & 7.4 & -10.41 & 0.9 \\ 
  Ozone fold4 & 3 & 19 & 9.36 & -4.76 & 0.92 \\ 
  Ozone fold5 & 2 & 3 & 8.51 & -7.12 & 0.88 \\ 
  Servo fold1 & 12 & 5 & 0.31 & -2.83 & 0.89 \\ 
  Servo fold2 & 9 & 16 & 0.11 & -6.78 & 0.97 \\ 
  Servo fold3 & 11 & 2 & 0.87 & -8.84 & 0.97 \\ 
  Servo fold4 & 11 & 34 & 0.12 & -3.22 & 0.87 \\ 
  Servo fold5 & 11 & 33 & 0.12 & -3.22 & 0.87 \\ 
  Abalone & 1 & 150 & 0.13 & -6.25 & 0.92 \\ 
  autos & 5 & 18 & 0.8 & -8.44 & 0.92 \\ 
  bike & 8 & 23 & 0.11 & -6.78 & 0.97 \\ 
  artificial LM 128 & 2 & 17 & 9.47 & -6.41 & 0.5 \\ 
  artificial LM 256 & 3 & 50 & 5.57 & -8.71 & 0.52 \\ 
  artificial LM 512 & 2 & 16 & 0.19 & -2.78 & 0.51 \\ 
  artificial LM 1024 & 4 & 3 & 0.18 & -2.82 & 0.63 \\ 
  artificial LM 2048 & 9 & 17 & 0.23 & -3.86 & 0.91 \\ 
   Step  128 & 8 & 9 & 9.29 & -8.39 & 0.92 \\ 
   Step  256 & 9 & 30 & 0.3 & -7.36 & 0.77 \\ 
   Step  512 & 8 & 47 & 0.28 & -12.75 & 0.89 \\ 
   Step  1024 & 5 & 27 & 0.31 & -18.42 & 0.73 \\ 
   StepLinear  128 & 10 & 5 & 0.31 & -2.83 & 0.89 \\ 
   StepLinear  256 & 10 & 10 & 8.74 & -3 & 0.92 \\ 
   StepLinear  512 & 10 & 11 & 8.74 & -3 & 0.92 \\ 
   StepLinear  1024 & 10 & 12 & 8.74 & -3 & 0.92 \\ 
   \hline
\end{tabular}
\caption{The table summarizes the selected hyperparameters for the data sets described in Section \ref{sec:realworlddatasets}.} 
\label{tbl:hyperparameters}
\end{flushleft}
\end{table}


==> tables/performanceTables.tex <==
% latex table generated in R 3.5.3 by xtable 1.84 package
% Sat May 25 14:46:14 2019
\begin{table}[ht]
\begin{flushleft}
\begin{tabular}{rrrrrrrrr}
  \hline
 & RF & RF & RLM & BART & Cubist & RCART & local RF & Ridge RF \\ 
  \hline
 & forestry & ranger & glmnet & dbarts & Cubist & forestry & grf & forestry \\ 
  Abalone & 2.13 & 2.13 & 2.3 & 2.12 & 2.13 & 2.12 & \textbf{2.09} & 2.1 \\ 
  autos &  & 2389.33 & 3390.75 & 2385.69 & 2556.72 & 2780.74 & 3235.87 & \textbf{2364.98} \\ 
  bike & 74.11 & 71.85 & 144.46 & \textbf{58.57} & 63.15 & 76.49 & 69.38 & 61.01 \\ 
  Boston &  & 3.27 & 5.24 & \textbf{2.95} & 3.2 & 5.13 & 3.09 & 3.51 \\ 
  Friedman 1 & 1.91 & 1.9 & 2.72 & \textbf{1.21} & 1.24 & 1.45 & 1.9 & 1.26 \\ 
  Friedman 2 & 595.95 & 596.1 & 953.33 & 630.97 & \textbf{586.69} & 601.39 & 594.38 & 587.84 \\ 
  Friedman 3 & 0.32 & 0.32 & 0.37 & \textbf{0.32} & 0.32 & 0.32 & 0.32 & 0.32 \\ 
  Ozone & \textbf{4.03} & 4.04 & 4.72 & 4.12 & 4.4 & 4.61 & 4.14 & 4.04 \\ 
  Servo & 0.55 & 0.5 & 1.18 & 0.58 & 0.64 & 0.8 & \textbf{0.41} & 0.51 \\ 
   \hline
\end{tabular}
\caption{Performance of the estimators.} 
\label{tbl:performance}
\end{flushleft}
\end{table}



